Domain Knowledge Matters: Improving Prompts with Fix Templates for Repairing Python Type Errors

Although the dynamic type system of Python facilitates the developers in writing Python programs, it also brings type errors at run-time. There exist rule-based approaches for automatically repairing Python type errors. The approaches can generate accurate patches but they require domain experts to design patch synthesis rules and suffer from low template coverage of real-world type errors. Learning-based approaches alleviate the manual efforts in designing patch synthesis rules. Among the learning-based approaches, the prompt-based approach which leverages the knowledge base of code pre-trained models via pre-defined prompts, obtains state-of-the-art performance in general program repair tasks. However, such prompts are manually defined and do not involve any specific clues for repairing Python type errors, resulting in limited effectiveness. How to automatically improve prompts with the domain knowledge for type error repair is challenging yet under-explored. In this paper, we present TypeFix, a novel prompt-based approach with fix templates incorporated for repairing Python type errors. TypeFix first mines generalized fix templates via a novel hierarchical clustering algorithm. The identified fix templates indicate the common edit patterns and contexts of existing type error fixes. TypeFix then generates code prompts for code pre-trained models by employing the generalized fix templates as domain knowledge, in which the masks are adaptively located for each type error instead of being pre-determined. Experiments on two benchmarks, including BugsInPy and TypeBugs, show that TypeFix successfully repairs 26 and 55 type errors, outperforming the best baseline approach by 9 and 14, respectively. Besides, the proposed fix template mining approach can cover 75% of developers' patches in both benchmarks, increasing the best rule-based approach PyTER by more than 30%.

==> tables/dataset.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Statistics of Two Benchmarks}
    \label{tab:dataset}
\end{table}

==> tables/motex.tex <==
\begin{table}[t]
    \centering
    \caption{Patches provided by current approaches and \tool.}
    \begin{tabular}{ccc}
    \toprule
        \textbf{Approach} &  \textbf{Correct?} & \textbf{Patch} \\
    \midrule
        AlphaRepair & No & \\
        CoCoNut & No & \\
        Codex & No & 
\begin{lstlisting} 
if not isinstance(user, bytes):
    user = user.encode('ascii')
if not isinstance(password, bytes):
    password = password.encode('ascii')
\end{lstlisting} \\
        PyTER & No & \\
       \tool  & Yes &  Identical to developer fix \\
    \bottomrule
    \end{tabular}
    \label{tab:motex}
\end{table}

==> tables/short_mainres.tex <==
\begin{table*}[t]
    \centering
    \caption{Evaluation results of \tool compared with three baselines. Results are presented in the Correct/Plausible format. The number highlighted in \colorbox{mygray}{gray} for \tool and PyTER represents the Template Match metric. }
    \scalebox{1.0}{
    \begin{tabular}{cc|cccc}
    \toprule
        \multicolumn{6}{c}{\g \textbf{\textsc{TypeBugs}}} \\
        \midrule
         & \textbf{\#Bug}& \textbf{\tool} & \textbf{PyTER} & \textbf{AlphaRepair} & \textbf{CoCoNuT}\\
        \midrule
        \textbf{Total}  & 109 & 55/76 & 41/60 &  19/46 & 5/21\\
        \textbf{Rate (\%)} & - & 50.5/70.0 & 37.6/55.0 & 17.4/42.2 & 4.6/19.3\\
        \midrule
        \multicolumn{6}{c}{\g \textbf{\textsc{BugsInPy}}} \\
        \midrule
         & \textbf{\#Bug} & \textbf{\tool} & \textbf{PyTER} & \textbf{AlphaRepair} & \textbf{CoCoNuT} \\
        \midrule
        \textbf{Total} & 54 & 26/41 & 15/26  & 6/21 & 7/19\\
        \textbf{Rate (\%)} & - & 48.1/76.0 & 27.8/48.1  & 11.1/38.9 & 13.0/35.2\\
    \bottomrule
    \end{tabular}}
    \label{tab:short_main_res}
\end{table*}
